Learning to Rank Anomalies: Scalar Performance Criteria and Maximization of Two-Sample Rank Statistics

The ability to collect and store ever more massive databases has been accompanied by the need to process them efficiently. In many cases, most observations have the same behavior, while a probable small proportion of these observations are abnormal. Detecting the latter, defined as outliers, is one of the major challenges for machine learning applications (e.g. in fraud detection or in predictive maintenance). In this paper, we propose a methodology addressing the problem of outlier detection, by learning a data-driven scoring function defined on the feature space which reflects the degree of abnormality of the observations. This scoring function is learnt through a well-designed binary classification problem whose empirical criterion takes the form of a two-sample linear rank statistics on which theoretical results are available. We illustrate our methodology with preliminary encouraging numerical experiments.

==> algorithm.tex <==

We present two learning algorithms adopted in this framework to estimate the optimal empirical scoring function, as the empirical maximizer of the $W_{\phi}$-performance criterion, that provides a ranking rule for the probable \textit{anomalous} sample, following steps $1$ and $2$ as presented in \ref{sub:meth_proc}. 



We first present an 'exact' algorithm that exactly maximizes the criterion we introduced, such that the $\roc^*$ is recovered and that allows to maximize the former for all the choices of score-generating functions. This method is based on the grounded results in \cite{CleLimVay21}, when assuming a parametric class of scoring functions $\S_{\Theta}$, say $\Theta \in \Z$ is the parameter space, that is constructed via a vanilla gradient ascent \wrt to the space $\Theta$ and that optimizes a smoothed version of the statistic. In particular, for some choices of probability functions and scoring classes, we can ensure to avoid the approximation error.\\

The second learning algorithm is based on a $2$-layer Neural Net, where the loss function is $	\widehat{W}_{n,m}^{\phi}$.


 %We propose two different algorithms based on  We first point out that the optimization of the empirical criterion \eqref{def:R_stat} is of high computational complexity, of order $O(N^2)$

